Incremental Few-Shot Learning with Attention Attractor Networks

Machine learning classifiers are often trained to recognize a set of pre-defined classes. However, in many applications, it is often desirable to have the flexibility of learning additional concepts, with limited data and without re-training on the full training set. This paper addresses this problem, incremental few-shot learning, where a regular classification network has already been trained to recognize a set of base classes, and several extra novel classes are being considered, each with only a few labeled examples. After learning the novel classes, the model is then evaluated on the overall classification performance on both base and novel classes. To this end, we propose a meta-learning model, the Attention Attractor Network, which regularizes the learning of novel classes. In each episode, we train a set of new weights to recognize novel classes until they converge, and we show that the technique of recurrent back-propagation can back-propagate through the optimization process and facilitate the learning of these parameters. We demonstrate that the learned attractor network can help recognize novel classes while remembering old classes without the need to review the original training set, outperforming various baselines.

==> sections/dataset_stats.tex <==
% % !TEX root = ../main.tex
% \begin{table}[h]
% \begin{small}
% \caption{\textit{mini}-ImageNet and \textit{tiered}-ImageNet split statistics}
% \label{tab:stats}
% \begin{center}
% \begin{tabular}{cc|crr|crr}
% && \multicolumn{3}{c|}{\textit{mini}-ImageNet}& \multicolumn{3}{c}{\textit{tiered}-ImageNet} \\
% Classes                & Purpose & Split         & N. Cls  & N. Img  & Split           & N. Cls   & N. Img \\
% \hline
% \hline
% \multirow{3}{*}{Base}  & Train   & Train-Train   & 64      & 38,400  & Train-A-Train   & 200      & 203,751   \\
%                       & Val     & Train-Val     & 64      & 18,748  & Train-A-Val     & 200      & 25,460    \\
%                       & Test    & Train-Test    & 64      & 19,200  & Train-A-Test    & 200      & 25,488    \\
% \hline
% \multirow{3}{*}{Novel} & Train   & Train-Train   & 64      & 38,400  & Train-B         & 151      & 193,996   \\
%                       & Val     & Val           & 16      & 9,600   & Val             & 97       & 124,261   \\
%                       & Test    & Test          & 20      & 12,000  & Test            & 160      & 206,209   \\
% \end{tabular}
% \end{center}
% \end{small}
% \end{table}


==> sections/table_bptt.tex <==
% !TEX root = ../main.tex
% \begin{table*}[t]
% \begin{small}
% \begin{center}
% \caption{Learning an attention attractor network using damped Neumann RBP vs. truncated BPTT. Models
% are on evaluated on the validation set of \textit{tiered}-ImageNet. During evaluation, ``*'' models
% are solved till convergence using a second-order optimizer.}
% \label{tab:bptt}
% \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{l|ccc|ccc|cc}
% \hline\hline
% 1-shot           & Base & Base+ & $\Delta_a$& Novel & Novel+ & $\Delta_b$ & Both& $\overline{\Delta}$ \\
% \hline\hline
% BPTT 20 Steps    & 61.99 & 61.35 & -0.64              & 50.98 $\pm$ 0.46 & 49.37 $\pm$ 0.45 &-1.61&                        55.36 & -1.12   \\
% BPTT 100 Steps   & 61.96 & 61.66 & -0.31              & 53.26 $\pm$ 0.47 & 52.10 $\pm$ 0.46 &-0.73&                        56.87 & -2.20   \\
% BPTT 200 Steps   & 62.13 & 61.42 & -0.70              & 53.93 $\pm$ 0.46 & 53.02 $\pm$ 0.46 &-0.81&                        57.22 & -1.83   \\
% \hline
% BPTT 20 Steps *  & 61.98 & 14.22 & \color{red}{-47.76}& 32.53 $\pm$ 0.38 & 32.53 $\pm$ 0.38 &-0.00&\color{red}{23.38}&\color{red}{-23.88} \\
% BPTT 100 Steps * & 62.22 & 26.03  & \color{red}{-36.19}& 35.77 $\pm$ 0.40 & 35.76 $\pm$ 0.40 &-0.01&\color{red}{30.90}&\color{red}{-18.10} \\
% BPTT 200 Steps * & 62.19 & 34.93  & \color{red}{-27.26}&36.87$\pm$  0.42& 36.81 $\pm$ 0.42 &  -0.06 & \color{red}{35.87} & \color{red}{-13.66} \\
% \hline
% Ours (RBP 20 Steps) & 61.99 & 61.74 & -0.25 & 55.99 $\pm$ 0.46 & 55.52 $\pm$ 0.46 & -0.47  & \textbf{58.63} & \textbf{-0.36}
% \end{tabular}
% }
% \vspace{-0.2in}
% % \newline
% \iffalse
% \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{l|ccc|ccc|cc}
% \hline\hline
% 5-shot           & Base & Base+ & $\Delta_a$& Novel & Novel+ & $\Delta_b$ & Both& $\overline{\Delta}$ \\
% \hline\hline
% BPTT 20 Steps    & 61.78 & 61.58 & -0.21              &67.63 $\pm$ 0.40& 66.67 $\pm$ 0.39 & -0.96 & 64.12 & -0.58 \\
% BPTT 100 Steps   & 62.10 & 61.47 & -0.63              &71.77 $\pm$ 0.37& 71.31 $\pm$ 0.36 & -0.46 & 66.39 & -0.54 \\
% BPTT 200 Steps   & 62.10 & 61.54 & -0.56              &71.87 $\pm$ 0.39& 71.52 $\pm$ 0.39 & -0.35 & 66.53 & -0.45 \\
% \hline
% BPTT 20 Steps *  & 62.12 & 5.50  & \color{red}{-56.68}&53.06 $\pm$ 0.42& 53.06 $\pm$ 0.42 & -0.00 & \color{red}{29.28} & \color{red}{-28.34} \\
% BPTT 100 Steps * & 62.18 & 8.09  & \color{red}{-54.09}&50.03$\pm$  0.39& 50.03 $\pm$ 0.39 &  -0.00 & \color{red}{29.06} & \color{red}{-27.04} \\
% BPTT 200 Steps * & 62.29 & 29.48  & \color{red}{-32.81}&44.14$\pm$  0.36& 44.09 $\pm$ 0.37 &  -0.05 & \color{red}{36.79} & \color{red}{-16.43} \\
% \hline
% Ours (RBP 20 Steps) & 61.99 & 61.83 & -0.16 & 71.69 $\pm$ 0.39 & 71.38 $\pm$ 0.39 & -0.31  & \textbf{66.60} & \textbf{-0.24}
% \end{tabular}
% }
% \fi
% \end{center}
% \end{small}
% \end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}[t]
% \begin{small}
% \begin{center}
% \caption{Learning an attention attractor network using damped Neumann RBP vs. truncated BPTT. Models
% are on evaluated on the validation set of \textit{tiered}-ImageNet. During evaluation, ``*'' models
% are solved till convergence using a second-order optimizer.}
% \label{tab:bptt}
% % \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{l|cc}
% \hline\hline
% 1-shot & Both & $\overline{\Delta}$ \\
% \hline\hline
% BPTT 20 Steps    & 55.36 & -1.12   \\
% BPTT 100 Steps   & 56.87 & -2.20   \\
% BPTT 200 Steps   & 57.22 & -1.83   \\
% \hline
% BPTT 20 Steps *  & \color{red}{23.38} & \color{red}{-23.88} \\
% BPTT 100 Steps * & \color{red}{30.90} & \color{red}{-18.10} \\
% BPTT 200 Steps * & \color{red}{35.87} & \color{red}{-13.66} \\
% \hline
% Ours (RBP 20 Steps) & \textbf{58.63} & \textbf{-0.36}
% \end{tabular}
% % }
% \vspace{-0.2in}
% % \newline
% \end{center}
% \end{small}
% \end{table}


==> sections/table_fullresults.tex <==
% !TEX root = ../supp.tex
\begin{table}[H]
\centering
\small
\caption{Full ablation results on 64+5-way {\it mini}-ImageNet}
\label{tab:full1}
% \resizebox{0.8\textwidth}{!}{
\begin{tabular}{c|cccc|cccc}
% \hline
\toprule
          & \multicolumn{4}{c|}{1-shot}           & \multicolumn{4}{c}{5-shot} \\
          & Acc. $\ua$            & \D         & \Da    &\Db     & Acc. $\ua$            & \D         & \Da    & \Db     \\
% \hline\hline       
\midrule                                                                                                         
LR        & 52.74 $\pm$ 0.24      & -13.95     & -8.98  & -24.32 & 60.34 $\pm$ 0.20      & -13.60     & -10.81 & -15.97  \\
LR +S     & 53.63 $\pm$ 0.30      & -12.53     & -9.44  & -15.62 & 62.50 $\pm$ 0.30      & -11.29     & -13.84 & -8.75   \\
LR +A     & \tb{55.31} $\pm$ 0.32 & \tb{-11.72}& -12.72 & -10.71  & 63.00 $\pm$ 0.29      & -10.80     & -13.59 & -8.01   \\
% \hline      
\midrule                                                                                                                        
MLP       & 49.36 $\pm$ 0.29      & -16.78     & -8.95  & -24.61 & 60.85 $\pm$ 0.29      & -12.62     & -11.35 & -13.89  \\
MLP +S    & 54.46 $\pm$ 0.31      & -11.74     & -12.73 & -10.74 & 62.79 $\pm$ 0.31      & -10.77     & -12.61 & -8.80   \\
MLP +A    & 54.95 $\pm$ 0.30      & -11.84     & -12.81 & -10.87 & \tb{63.04} $\pm$ 0.30 & \tb{-10.66}& -12.55 & -8.77   \\
% \hline
\bottomrule
\end{tabular}
% }
\end{table}

\begin{table}[H]
\centering
\caption{Full ablation results on 200+5-way {\it tiered}-ImageNet}
\label{tab:full2}
% \resizebox{0.8\textwidth}{!}{
\begin{tabular}{c|cccc|cccc}
% \hline
\toprule
          & \multicolumn{4}{c|}{1-shot}           & \multicolumn{4}{c}{5-shot} \\
          & Acc. $\ua$            & \D         & \Da    & \Db    & Acc. $\ua$            & \D         & \Da    & \Db     \\
% \hline\hline
\midrule                                                                                                              
LR        & 48.84 $\pm$ 0.23      & -10.44     & -11.65 & -9.24  & 62.08 $\pm$ 0.20      & -8.00      & -5.49  & -10.51  \\
LR +S     & 55.36 $\pm$ 0.32      & -6.88      & -7.21  & -6.55  & 65.53 $\pm$ 0.30      & -4.68      & -4.72  & -4.63   \\
LR +A     & 55.98 $\pm$ 0.32      & \tb{-6.07} & -6.64  & -5.51  & 65.58 $\pm$ 0.29      & \tb{-4.39} & -4.87  & -3.91   \\
% \hline     
\midrule                                                                                                                                        
MLP       & 41.22 $\pm$ 0.35      & -10.61     & -11.25 & -9.98  & 62.70 $\pm$ 0.31      & -7.44      & -6.05  & -8.82   \\
MLP +S    & \tb{56.16} $\pm$ 0.32 & -6.28      & -6.83  & -5.73  & \tb{65.80} $\pm$ 0.31 & -4.58      & -4.66  & -4.51   \\
MLP +A    & 56.11 $\pm$ 0.33      & 6.11       & -6.79  & -5.43  & 65.52 $\pm$ 0.31      & -4.48      & -4.91  & -4.05   \\
% \hline
\bottomrule
\end{tabular}
% }
\end{table}

==> sections/table_split.tex <==
% !TEX root = ../main.tex
\begin{table*}[ht]
\vspace{-0.15in}
\begin{small}
\caption{\textit{mini}-ImageNet and \textit{tiered}-ImageNet split statistics}
\label{tab:stats}
\begin{center}
\resizebox{0.75\columnwidth}{!}{
\begin{tabular}{|cc|crr|crr|}
\hline
&& \multicolumn{3}{c|}{\textit{mini}-ImageNet}& \multicolumn{3}{c|}{\textit{tiered}-ImageNet} \\
Classes                & Purpose & Split         & N. Cls  & N. Img  & Split           & N. Cls   & N. Img \\
\hline
\hline
\multirow{3}{*}{Base}  & Train   & Train-Train   & 64      & 38,400  & Train-A-Train   & 200      & 203,751   \\
                       & Val     & Train-Val     & 64      & 18,748  & Train-A-Val     & 200      & 25,460    \\
                       & Test    & Train-Test    & 64      & 19,200  & Train-A-Test    & 200      & 25,488    \\
\hline
\multirow{3}{*}{Novel} & Train   & Train-Train   & 64      & 38,400  & Train-B         & 151      & 193,996   \\
                       & Val     & Val           & 16      & 9,600   & Val             & 97       & 124,261   \\
                       & Test    & Test          & 20      & 12,000  & Test            & 160      & 206,209   \\
\hline
\end{tabular}
}
\end{center}
\end{small}
\vspace{-0.2in}
\end{table*}

